Cascade-CLIP: Cascaded Vision-Language Embeddings Alignment for Zero-Shot Semantic Segmentation

Pre-trained vision-language models, e.g., CLIP, have been successfully applied to zero-shot semantic segmentation. Existing CLIP-based approaches primarily utilize visual features from the last layer to align with text embeddings, while they neglect the crucial information in intermediate layers that contain rich object details. However, we find that directly aggregating the multi-level visual features weakens the zero-shot ability for novel classes. The large differences between the visual features from different layers make these features hard to align well with the text embeddings. We resolve this problem by introducing a series of independent decoders to align the multi-level visual features with the text embeddings in a cascaded way, forming a novel but simple framework named Cascade-CLIP. Our Cascade-CLIP is flexible and can be easily applied to existing zero-shot semantic segmentation methods. Experimental results show that our simple Cascade-CLIP achieves superior zero-shot performance on segmentation benchmarks, like COCO-Stuff, Pascal-VOC, and Pascal-Context. Our code is available at: https://github.com/HVision-NKU/Cascade-CLIP

==> figs/A-visualisation_inductive.tex <==
\begin{figure*}[!t]
\centering
    \vspace{5pt}
    \begin{minipage}[t]{0.8\linewidth}
        \centering
        \begin{overpic}[width=1\textwidth]{A-visualisation_inductive-1}
        \put(5,37.5){\footnotesize{Origin Image}}
        \put(29,37.5){\footnotesize{layer 12}}
        \put(49,37.5){\footnotesize{layer 11}}
        \put(69,37.5){\footnotesize{layer 8}}
        \put(88,37.5){\footnotesize{layer 5}}
        % \put(0,17){\dashline{3 3}(100,0)}
        \put(0,20){\tikz\draw[dashed,line width = 0.5pt](0,0)--(13.7,0);}

        \put(5,16.5){\footnotesize{Ground Truth}}
        \put(32,16.5){\footnotesize{Fusion \{12\}}}
        \put(54,16.5){\footnotesize{Fusion \{9-11, 12\}}}
        \put(77.5,16.5){\footnotesize{Fusion \{6-8, 9-11, 12\}}}

        \put(0,-2){\line(1,0){100}}

        \end{overpic}
    \end{minipage}
    % \vspace{10pt}
    % \\
    % \begin{minipage}[t]{0.8\linewidth}
    % \centering
    % \begin{overpic}[width=1\textwidth]{A-visualisation_inductive-2}
    %     \put(0,18.5){\tikz\draw[dashed,line width = 0.5pt](0,0)--(13.7,0);}
    %     \put(0,-2){\line(1,0){100}} 
    % \end{overpic}
    % \end{minipage}   
    \vspace{10pt}
    \\
    \begin{minipage}[t]{0.8\linewidth}
    \centering
    \begin{overpic}[width=1\textwidth]{A-visualisation_inductive-3}
        \put(0,16.5){\tikz\draw[dashed,line width = 0.5pt](0,0)--(13.7,0);}
        % \put(0,-2){\line(1,0){100}}
    \end{overpic}
    \end{minipage}   
    % \vspace{10pt}
    % \\
    % \begin{minipage}[t]{0.8\linewidth}
    % \centering
    % \begin{overpic}[width=1\textwidth]{A-visualisation_inductive-4} 
    %     \put(0,18.5){\tikz\draw[dashed,line width = 0.5pt](0,0)--(13.7,0);}
    % \end{overpic}
    % \end{minipage}   
    % \vspace{5pt}
\caption{Visualization of cosine similarity map about features and qualitative segmentation results.
% 
We visualize feature correspondence through cosine similarity calculations on visual patches of \textbf{unseen} classes from both deep and shallow layers in our \ourMthd~(above).
% 
The inductive segmentation results are generated by cascading different decoders~(bottom).
}
\label{A-visualisation_inductive}
\vskip -0.1in
\end{figure*}

==> figs/image_cosine_similarity.tex <==

% \begin{figure}[t]
%     \centering
%       \begin{overpic}[width=0.45\textwidth]{image_cosine_similarity}
%       \put(0,0){\footnotesize{\color{red} Cascaded}}
%       \end{overpic}
%      \vspace{5pt}
%     \caption{  }
%     \label{1-Introduction}
%   \end{figure}

\begin{figure*}[t]
\centering
    \vspace{6pt}
    \begin{overpic}[width=0.95\textwidth]{image_cosine_similarity2}
    \put(3,17.5){\footnotesize{Origin Image}}
    \put(21.5,17.5){\footnotesize{Layer 12}}
    \put(37.5,17.5){\footnotesize{Layer 11}}
    \put(54.5,17.5){\footnotesize{Layer 9}}
    \put(71.5,17.5){\footnotesize{Layer 6}}
    \put(88.5,17.5){\footnotesize{Layer 3}}
    \end{overpic}
    % \vspace{1pt}
\caption{Visualisation of feature correspondence by computing the cosine similarity of different visual patch tokens 
extracted from the various layers of pre-trained CLIP~\cite{pmlr-v139-radford21a}.}
\label{Image_cosine_similarity}
\end{figure*}

==> figs/text_image_sim.tex <==

\begin{figure}[!t]
\centering
    \vspace{5pt}
    \begin{overpic}[width=0.46\textwidth]{text_image_sim}
    \put(-3,15){\rotatebox[]{-90}{\footnotesize{Probabilities}}}
    \put(45,-2.5){\footnotesize{Unseen Class}}
    \end{overpic}
    \vspace{7pt}
\caption{   }
\label{text_image_sim}
\end{figure}

==> figs/visualisation_inductive.tex <==
\begin{figure*}[t]
\centering
    \vspace{10pt}
    % \begin{minipage}[t]{0.95\linewidth}
    %     \centering
    %     \begin{overpic}[width=0.95\textwidth]{visualisation_inductive1}
    %         \put(17,9){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize clouds}}}
    %         \put(33.8,9){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize clouds}}}
    %         \put(50.5,9){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize clouds}}}
    %         \put(67.3,9){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize clouds}}}
    %         \put(84,9){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize clouds}}}
    
    %         \put(17,2){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize sea}}}    
    %         \put(33.8,2){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize sea}}}    
    %         \put(50.5,2){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize sea}}}    
    %         \put(67.3,2){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize sea}}}    
    %         \put(84,2){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize sea}}}   

    %         \put(18,6){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize person}}}    
    %         \put(34.8,6){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize person}}}    
    %         \put(51.5,6){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize person}}}    
    %         \put(68.3,6){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize person}}}    
    %         \put(85,6){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize person}}}    

    %         \put(25,1){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize surfboard}}}    
    %         \put(41.8,1){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize surfboard}}}    
    %         \put(58.5,1){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize surfboard}}}    
    %         \put(75.3,1){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize surfboard}}}    
    %         \put(92,1){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize surfboard}}}    

    %         \put(25.5,8){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize mountain}}}    
    %         \put(42.3,8){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize mountain}}}    
    %         \put(59,8){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize mountain}}}    
    %         \put(75.8,8){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize mountain}}}    
    %         \put(92.5,8){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize mountain}}}    
    %     \end{overpic}
    % \end{minipage}
    % \\
    % \vspace{5pt}
    % \\
    \begin{minipage}[t]{0.95\linewidth}
        \centering
        \begin{overpic}[width=0.95\textwidth]{visualisation_inductive2}
            \put(17,8.5){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize tree}}}
            \put(33.8,8.5){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize tree}}}
            \put(50.5,8.5){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize tree}}}
            \put(67.3,8.5){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize tree}}}
            \put(84,8.5){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize tree}}}

            \put(17,5){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize person}}}    
            \put(33.8,5){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize person}}}    
            \put(50.5,5){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize person}}}    
            \put(67.3,5){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize person}}}    
            \put(84,5){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize person}}}    
            
            \put(27,9){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize sky}}}    
            \put(43.8,9){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize sky}}}    
            \put(60.5,9){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize sky}}}    
            \put(77,9){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize sky}}}    
            \put(94,9){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize sky}}}   
            
            \put(24,6){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize giraffe}}}
            \put(40.8,6){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize giraffe}}}
            \put(57.5,6){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize giraffe}}}
            \put(74,6){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize giraffe}}}
            \put(91,6){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize giraffe}}}

        \end{overpic}
    \end{minipage}
        \vspace{3pt}
        \\
        \begin{minipage}[t]{0.95\linewidth}
            \centering
            \begin{overpic}[width=0.95\textwidth]{visualisation_inductive3}
                \put(17,10){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize playing field}}}
                \put(33.8,10){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize playing field}}}
                \put(50.5,10){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize playing field}}}
                \put(67.3,10){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize playing field}}}
                \put(84,10){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize playing field}}}
    
                \put(17,5){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize person}}}    
                \put(33.8,5){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize person}}}    
                \put(50.5,5){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize person}}}    
                \put(67.3,5){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize person}}}    
                \put(84,5){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize person}}}    
                
                % \put(27,9){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize sky}}}    
                \put(45.8,1){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize dirt}}}    
                \put(62.5,1){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize dirt}}}    
                \put(79,1){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize dirt}}}    
                \put(96,1){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize dirt}}}   
                

                \put(42.8,5){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize glove}}}    
                \put(59.5,5){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize glove}}}    
                \put(76.5,5){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize glove}}}    
                \put(93.8,5){\transparent{0.7}\colorbox{white}{\textcolor{black}{\scriptsize glove}}}    

                % \put(24,6){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize giraffe}}}
                % \put(40.8,6){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize giraffe}}}
                % \put(57.5,6){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize giraffe}}}
                % \put(74,6){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize giraffe}}}
                % \put(91,6){\transparent{0.7}\colorbox{white}{\textcolor{red}{\scriptsize giraffe}}}
                
                
                \put(3,-2){{\scriptsize (a) Origin Image}}
                \put(20,-2){{\scriptsize (b) Ground truth}}
                \put(39,-2){{\scriptsize (c) \ourMthd}}
                \put(54,-2){{\scriptsize (d) \ourMthd~wo/S1}}
                \put(70,-2){{\scriptsize (e) \ourMthd~wo/S2}}
                \put(87,-2){{\scriptsize (f) \ourMthd~wo/S3}}





            \end{overpic}
    \end{minipage}
    \vspace{1pt}
\caption{   }
\label{visualisation_inductive}
\end{figure*}

==> tabs/sota-transductive.tex <==
\begin{table*}[t]
    \centering
    \vskip -0.15in
    \caption{Comparison with the \emph{\textbf{transductive}} state-of-the-art zero-shot segmentation methods on COCO-Stuff 164K, and PASCAL VOC 2012 datasets.
    mIoU$^S$ and mIoU$^U$ denote the mIoU(\%) of seen classes and unseen classes, respectively.
    }
    \label{tab: sota-transductive}
%\vskip 0.15in
    \begin{center}
    \begin{small}
    % \begin{sc}
    \setlength{\tabcolsep}{1.0mm}{
    \begin{tabular}{ccccccccccc}
    \toprule
    \multirow{2}{*}{Methods}& \multirow{2}{*}{Backbone} & \multirow{2}{*}{Segmentor}& \multicolumn{3}{c}{COCO-Stuff 164K~(171)}&\multicolumn{3}{c}{PASCAL VOC 2012~(20)} \\  
    \cmidrule(lr){4-6}  \cmidrule(lr){7-9}
     & &  & mIoU$^S$$\uparrow$& mIoU$^U$$\uparrow$& hIoU$\uparrow$& mIoU$^S$$\uparrow$& mIoU$^U$$\uparrow$& hIoU$\uparrow$ \\
    \midrule
    \multicolumn{9}{l}{\emph{\textbf{Transductive: training images employ the names of unseen classes.}}} \\
    Zsseg+ST~\cite{xu2021simple}&R101\&CLIP-B& MaskFormer &39.6& 43.6& 41.5& 79.2& 78.1& 79.3\\
    FreeSeg~\cite{Qin_2023_CVPR}&R101\&CLIP-B& Mask2Former& 42.4& 42.2& 42.3&91.9 &78.6&84.7\\
    FreeSeg+MAFT~\cite{jiao2023learning}&R101\&CLIP-B& Mask2Former&44.1&55.2&49.0&90.0&86.3&88.1 \\
    SPNet-C+ST~\cite{xian2019semantic} & R101& W2V\&FT& 34.6& 26.9 & 30.3& 77.8& 25.8& 38.8 \\
    ZS5Net~\cite{bucher2019zero}  & R101& W2V    & 34.9& 10.6 & 16.2& 78.0& 21.2& 33.3 \\
    CaGNet+ST~\cite{gu2020context}   & R101& W2V\&FT& 35.6& 13.4& 19.5& 78.6& 30.3& 43.7 \\
    % \midrule 
    MaskCLIP$\textbf{\textbf{+}}$~\cite{zhou2022extract}  & R101 & DeepLabv2& 38.1& 54.7& 45.0& 88.8& 86.1& 87.4\\
    ZegCLIP+ST~\cite{Zhou_2023_CVPR}&CLIP-B &- &    40.7& 59.9& 48.5& 92.3& 89.9& 91.1 \\
    \ourMthd+ST (Ours) &CLIP-B &-&\textbf{41.7}& \textbf{62.5}& \textbf{50.0}& \textbf{93.3}& \textbf{93.4} & \textbf{93.4} \\
    % \midrule 
    % SPT~\cite{xu2023spectral}&CLIP-B &- & 40.4   &57.5 & 47.4 & 93.6& 92.2 & 92.9      \\
    % SPT+\ourMthd+ST&CLIP-B &- &\textbf{41.7}&\textbf{62.1}&\textbf{49.9}&\textbf{93.8}&\textbf{94.4}&\textbf{94.1}   \\
    % \midrule
    % \multicolumn{1}{l}{\emph{\textbf{Fully Supervised}}} \\
    % ZegCLIP~\cite{Zhou_2023_CVPR}&CLIP-B &- &40.7& 63.2& 49.6& 92.4& 90.9& 91.6 \\
    % \ourMthd&CLIP-B &- &41.3& 63.2& 50.0 & 93.7 & 94.6& 94.2\\
    \bottomrule
    \end{tabular}}
    % \end{sc}
    \end{small}
    \end{center}
    \vskip -0.1in
\end{table*}
